Curvature estimates for stable marginally trapped surfaces

We derive integral and sup-estimates for the curvature of stably marginally outer trapped surfaces in a sliced space-time. The estimates bound the shear of a marginally outer trapped surface in terms of the intrinsic and extrinsic curvature of a slice containing the surface. These estimates are well adapted to situations of physical insterest, such as dynamical horizons.

==> compact.tex <==
\section{A Compactness Property for MOTS}
\label{sec:compact}
% We are dealing with an alternative approach to the compactness
% theorem.
\begin{theorem}
Let $F_n : (\Sigma_n, \gamma_n, x_n) \to (M_n, g_n, p_n)$ be a sequence of
pointed isometric embeddings, ie. $F_n:\Sigma_n\to M_n$ satisfies
$F_n(p_n)=x_n$. Assume furthermore that 
\end{theorem}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "curv_est_omts"
%%% End: 


==> draft_commands.tex <==
%\usepackage{showtags}
%\usepackage[inner]{showlabels}
\input{svn_version}
\usepackage{margintext}
\usepackage{datetime}
\settimeformat{xxivtime}
\newdateformat{dashdate}{\twodigit{\THEYEAR}-\twodigit{\THEMONTH}-\twodigit{\THEDAY}}
\margintext{Rev: \svnversion\ \ \ Built: \dashdate\today\ \currenttime}


==> svn_version.tex <==
\newcommand{\svnversion}{%
357M
}

